3rd generation SUSY searches at CMS

The latest results on searches for stop and sbottom squarks are presented. Searches for direct squark production in a variety of decay channels are reviewed. The results are based on 19.5/fb of LHC proton-proton collisions at sqrt = 8 TeV taken with the CMS detector.

==> pdefs.tex <==
\def\Fileversion$#1: #2 ${\gdef\fileversion{#2}}
\def\Filedate$#1: #2-#3-#4 #5 ${\gdef\filedate{#2/#3/#4}}
\Fileversion$Revision: 259870 $
\Filedate$Date: 2014-09-10 19:11:09 +0200 (Wed, 10 Sep 2014) $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  CMS Common definitions style file
%
%  N.B. use of \newcommand rather than \newcommand means
%       that a definition is ignored if already specified
%
%                                              L. Taylor 18 Feb 2005
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{ptdr-definitions}[\filedate\space CMS Additional Macro Definitions (\fileversion)]
\RequirePackage{xspace}
\RequirePackage{amsmath}

% Some shorthand
% turn off italics
\newcommand {\etal}{\mbox{et al.}\xspace} %et al. - no preceding comma
\newcommand {\ie}{\mbox{i.e.}\xspace}     %i.e.
\newcommand {\eg}{\mbox{e.g.}\xspace}     %e.g.
\newcommand {\etc}{\mbox{etc.}\xspace}     %etc.
\newcommand {\vs}{\mbox{\sl vs.}\xspace}      %vs.
\newcommand {\mdash}{\ensuremath{\mathrm{-}}} % for use within formulas
\newcommand {\cmsSymbolFace}{\mathrm}

% some terms whose definition we may change
\newcommand {\Lone}{Level-1\xspace} % Level-1 or L1 ?
\newcommand {\Ltwo}{Level-2\xspace}
\newcommand {\Lthree}{Level-3\xspace}

% Some software programs (alphabetized)
\newcommand{\ACERMC} {\textsc{AcerMC}\xspace}
\newcommand{\ALPGEN} {{\textsc{alpgen}}\xspace}
\newcommand{\CALCHEP} {{\textsc{CalcHEP}}\xspace}
\newcommand{\CHARYBDIS} {{\textsc{charybdis}}\xspace}
\newcommand{\CMKIN} {\textsc{cmkin}\xspace}
\newcommand{\CMSIM} {{\textsc{cmsim}}\xspace}
\newcommand{\CMSSW} {{\textsc{cmssw}}\xspace}
\newcommand{\COBRA} {{\textsc{cobra}}\xspace}
\newcommand{\COCOA} {{\textsc{cocoa}}\xspace}
\newcommand{\COMPHEP} {\textsc{CompHEP}\xspace}
\newcommand{\EVTGEN} {{\textsc{evtgen}}\xspace}
\newcommand{\FAMOS} {{\textsc{famos}}\xspace}
\newcommand{\FEWZ} {{\textsc{fewz}}\xspace}
\newcommand{\GARCON} {\textsc{garcon}\xspace}
\newcommand{\GARFIELD} {{\textsc{garfield}}\xspace}
\newcommand{\GEANE} {{\textsc{geane}}\xspace}
\newcommand{\GEANTfour} {{\textsc{Geant4}}\xspace}
\newcommand{\GEANTthree} {{\textsc{geant3}}\xspace}
\newcommand{\GEANT} {{\textsc{geant}}\xspace}
\newcommand{\HDECAY} {\textsc{hdecay}\xspace}
\newcommand{\HERWIG} {{\textsc{herwig}}\xspace}
\newcommand{\HERWIGpp} {{\textsc{herwig++}}\xspace}
\newcommand{\POWHEG} {{\textsc{powheg}}\xspace}
\newcommand{\HIGLU} {{\textsc{higlu}}\xspace}
\newcommand{\HIJING} {{\textsc{hijing}}\xspace}
\newcommand{\IGUANA} {\textsc{iguana}\xspace}
\newcommand{\ISAJET} {{\textsc{isajet}}\xspace}
\newcommand{\ISAPYTHIA} {{\textsc{isapythia}}\xspace}
\newcommand{\ISASUGRA} {{\textsc{isasugra}}\xspace}
\newcommand{\ISASUSY} {{\textsc{isasusy}}\xspace}
\newcommand{\ISAWIG} {{\textsc{isawig}}\xspace}
\newcommand{\MADGRAPH} {\textsc{MadGraph}\xspace}
\newcommand{\MCATNLO} {\textsc{mc@nlo}\xspace}
\newcommand{\MCFM} {\textsc{mcfm}\xspace}
\newcommand{\MILLEPEDE} {{\textsc{millepede}}\xspace}
\newcommand{\ORCA} {{\textsc{orca}}\xspace}
\newcommand{\OSCAR} {{\textsc{oscar}}\xspace}
\newcommand{\PHOTOS} {\textsc{photos}\xspace}
\newcommand{\PROSPINO} {\textsc{prospino}\xspace}
\newcommand{\PYTHIA} {{\textsc{pythia}}\xspace}
\newcommand{\SHERPA} {{\textsc{sherpa}}\xspace}
\newcommand{\TAUOLA} {\textsc{tauola}\xspace}
\newcommand{\TOPREX} {\textsc{TopReX}\xspace}
\newcommand{\XDAQ} {{\textsc{xdaq}}\xspace}


%  Experiments
\newcommand {\DZERO}{D0\xspace}     %etc.


% Measurements and units...

\newcommand{\de}{\ensuremath{^\circ}}
\newcommand{\ten}[1]{\ensuremath{\times \text{10}^\text{#1}}}
\newcommand{\unit}[1]{\ensuremath{\text{\,#1}}\xspace}
\newcommand{\mum}{\ensuremath{\,\mu\text{m}}\xspace}
\newcommand{\micron}{\ensuremath{\,\mu\text{m}}\xspace}
\newcommand{\cm}{\ensuremath{\,\text{cm}}\xspace}
\newcommand{\mm}{\ensuremath{\,\text{mm}}\xspace}
\newcommand{\mus}{\ensuremath{\,\mu\text{s}}\xspace}
\newcommand{\keV}{\ensuremath{\,\text{ke\hspace{-.08em}V}}\xspace}
\newcommand{\MeV}{\ensuremath{\,\text{Me\hspace{-.08em}V}}\xspace}
\newcommand{\MeVns}{\ensuremath{\text{Me\hspace{-.08em}V}}\xspace} % no leading thinspace
\newcommand{\GeV}{\ensuremath{\,\text{Ge\hspace{-.08em}V}}\xspace}
\newcommand{\GeVns}{\ensuremath{\text{Ge\hspace{-.08em}V}}\xspace} % no leading thinspace
\newcommand{\gev}{\GeV}
\newcommand{\TeV}{\ensuremath{\,\text{Te\hspace{-.08em}V}}\xspace}
\newcommand{\TeVns}{\ensuremath{\text{Te\hspace{-.08em}V}}\xspace} % no leading thinspace
\newcommand{\PeV}{\ensuremath{\,\text{Pe\hspace{-.08em}V}}\xspace}
\newcommand{\keVc}{\ensuremath{{\,\text{ke\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c}}\xspace}
\newcommand{\MeVc}{\ensuremath{{\,\text{Me\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c}}\xspace}
\newcommand{\GeVc}{\ensuremath{{\,\text{Ge\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c}}\xspace}
\newcommand{\GeVcns}{\ensuremath{{\text{Ge\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c}}\xspace} % no leading thinspace
\newcommand{\TeVc}{\ensuremath{{\,\text{Te\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c}}\xspace}
\newcommand{\keVcc}{\ensuremath{{\,\text{ke\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c^\text{2}}}\xspace}
\newcommand{\MeVcc}{\ensuremath{{\,\text{Me\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c^\text{2}}}\xspace}
\newcommand{\GeVcc}{\ensuremath{{\,\text{Ge\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c^\text{2}}}\xspace}
\newcommand{\GeVccns}{\ensuremath{{\text{Ge\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c^\text{2}}}\xspace} % no leading thinspace
\newcommand{\TeVcc}{\ensuremath{{\,\text{Te\hspace{-.08em}V\hspace{-0.16em}/\hspace{-0.08em}}c^\text{2}}}\xspace}

\newcommand{\pbinv} {\mbox{\ensuremath{\,\text{pb}^\text{$-$1}}}\xspace}
\newcommand{\fbinv} {\mbox{\ensuremath{\,\text{fb}^\text{$-$1}}}\xspace}
\newcommand{\nbinv} {\mbox{\ensuremath{\,\text{nb}^\text{$-$1}}}\xspace}
\newcommand{\mubinv} {\ensuremath{\,\mu\mathrm{b}^{-1}}\xspace}
\newcommand{\percms}{\ensuremath{\,\text{cm}^\text{$-$2}\,\text{s}^\text{$-$1}}\xspace}
\newcommand{\lumi}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Lumi}{\ensuremath{\mathcal{L}}\xspace}%both upper and lower
%
% Need a convention here:
\newcommand{\LvLow}  {\ensuremath{\mathcal{L}=\text{10}^\text{32}\,\text{cm}^\text{$-$2}\,\text{s}^\text{$-$1}}\xspace}
\newcommand{\LLow}   {\ensuremath{\mathcal{L}=\text{10}^\text{33}\,\text{cm}^\text{$-$2}\,\text{s}^\text{$-$1}}\xspace}
\newcommand{\lowlumi}{\ensuremath{\mathcal{L}=\text{2}\times \text{10}^\text{33}\,\text{cm}^\text{$-$2}\,\text{s}^\text{$-$1}}\xspace}
\newcommand{\LMed}   {\ensuremath{\mathcal{L}=\text{2}\times \text{10}^\text{33}\,\text{cm}^\text{$-$2}\,\text{s}^\text{$-$1}}\xspace}
\newcommand{\LHigh}  {\ensuremath{\mathcal{L}=\text{10}^\text{34}\,\text{cm}^\text{$-$2}\,\text{s}^\text{$-$1}}\xspace}
\newcommand{\hilumi} {\ensuremath{\mathcal{L}=\text{10}^\text{34}\,\text{cm}^\text{$-$2}\,\text{s}^\text{$-$1}}\xspace}

% Physics symbols ...

\newcommand{\PT}{\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\ET}{\ensuremath{E_{\mathrm{T}}}\xspace}
\newcommand{\HT}{\ensuremath{H_{\mathrm{T}}}\xspace}
\newcommand{\et}{\ensuremath{E_{\mathrm{T}}}\xspace}
\newcommand{\Em}{\ensuremath{E\hspace{-0.6em}/}\xspace}
\newcommand{\Pm}{\ensuremath{p\hspace{-0.5em}/}\xspace}
\newcommand{\PTm}{\ensuremath{{p}_\mathrm{T}\hspace{-1.02em}/\kern 0.5em}\xspace}
\newcommand{\PTslash}{\PTm}
\newcommand{\ETm}{\ensuremath{E_{\mathrm{T}}^{\text{miss}}}\xspace}
\newcommand{\MET}{\ETm}
\newcommand{\ETmiss}{\ETm}
\newcommand{\ETslash}{\ensuremath{E_{\mathrm{T}}\hspace{-1.1em}/\kern0.45em}\xspace}
\newcommand{\VEtmiss}{\ensuremath{{\vec E}_{\mathrm{T}}^{\text{miss}}}\xspace}
\newcommand{\ptvec}{\ensuremath{{\vec p}_{\mathrm{T}}}\xspace}


% roman face derivative
\newcommand{\dd}[2]{\ensuremath{\frac{\cmsSymbolFace{d} #1}{\cmsSymbolFace{d} #2}}}
\newcommand{\ddinline}[2]{\ensuremath{\cmsSymbolFace{d} #1/\cmsSymbolFace{d} #2}}
\newcommand{\rd}{\ensuremath{\cmsSymbolFace{d}}}
\newcommand{\re}{\ensuremath{\cmsSymbolFace{e}}}
% absolute value
\newcommand{\abs}[1]{\ensuremath{\lvert #1 \rvert}}


\newcommand{\W}{\ensuremath{\mathrm{W}}\xspace}

\newcommand\defRTDR{\ensuremath{ R2 = \sqrt{[\pi-\Delta\phi(J_{1},\mht) ]^2 +[\Delta\phi(J_{2},\mht) ]^2}    }}
\newcommand\wpj{\ensuremath{\W + {\rm jets}}\xspace}
\newcommand\zpj{\ensuremath{\Z + {\rm jets}}\xspace}
\newcommand\qqbar{\ensuremath{{\rm q\bar{q}}}\xspace}
\newcommand{\ttbar}{\ensuremath{\cmsSymbolFace{t}\overline{\cmsSymbolFace{t}}}\xspace} % t-tbar
\newcommand\ttbarMuNu{\ensuremath{\ttbar ( \mu \nu ) {\rm +jets}}\xspace}
\newcommand\wtauhad{\ensuremath{\W \rightarrow \tau_{\rm h} \nu}\xspace}
\newcommand\ttbarTAUHNu{\ensuremath{\ttbar \rightarrow \tau_{\rm h} \nu + {\rm jets}}\xspace}
\newcommand\ttbarDITAUHNu{\ensuremath{\ttbar \rightarrow \tau_{\rm h} \nu + \tau_{\rm h} \nu + {\rm jets}}\xspace}
\newcommand\ttbarMUTAUHNu{\ensuremath{\ttbar ( \mu \nu + \tau_{\mu} \nu) {\rm +jets}}\xspace}
\newcommand\defMHT{\ensuremath{ {\rm MHT} = \mht = | - \sum_{i} \vec{p_{T} (jet_{i}) }|}}
\newcommand{\ztautau}{\ensuremath{\Z \rightarrow \tau \tau}\xspace}
\newcommand{\zmumu}{\ensuremath{\Z \rightarrow \mu^{+} \mu^{-}}\xspace}
\newcommand{\zee}{\ensuremath{\Z \rightarrow \e^{+} \e^{-}}\xspace}
\newcommand{\znunu}{\ensuremath{\Z \rightarrow \nu \bar{\nu}}\xspace}
\newcommand{\zll}{\ensuremath{\Z \rightarrow \ell^{+}\ell^{-}}\xspace}
\newcommand{\wlnu}{\ensuremath{\W \rightarrow \ell\nu}\xspace}
\newcommand{\wenu}{\ensuremath{\W \rightarrow \e\nu}\xspace}
\newcommand{\wmunu}{\ensuremath{\W \rightarrow \mu \nu}\xspace}
\newcommand{\zellell}{\ensuremath{\Z \rightarrow \ell^{+} \ell^{-}}\xspace}
\newcommand{\znunubr}{\ensuremath{\Z ( \nu \bar{\nu} )}\xspace}
\newcommand{\zellellbr}{\ensuremath{\Z ( \ell^{+} \ell^{-} )}\xspace}
\newcommand{\wmunubr}{\ensuremath{\W (\mu \nu )}\xspace}
\newcommand{\wenubr}{\ensuremath{\W (\e\nu )}\xspace}
\newcommand{\wlnubr}{\ensuremath{\W (\ell \nu )}\xspace}
\newcommand{\wellnubr}{\ensuremath{\W (\ell \nu )}\xspace}
\newcommand{\wtaunubr} {\ensuremath{\W (\tau \nu )}\xspace}
\newcommand{\ztautaubr}{\ensuremath{\Z (\tau \tau)}\xspace}
\newcommand{\zmumubr}  {\ensuremath{\Z (\mu \mu)}\xspace}
\newcommand{\zeebr}    {\ensuremath{\Z (\e \e)}\xspace}
\newcommand{\tauh}{\ensuremath{\tau_\mathrm{h}}\xspace}


%\ifthenelse{\boolean{cms@italic}}{\newcommand{\cmsSymbolFace}{\relax}}{\newcommand{\cmsSymbolFace}{\mathrm}}

% Particle names which track the italic/non-italic face convention
\newcommand{\zp}{\ensuremath{\cmsSymbolFace{Z}^\prime}\xspace} % plain Z'
\newcommand{\JPsi}{\ensuremath{\cmsSymbolFace{J}\hspace{-.08em}/\hspace{-.14em}\psi}\xspace} % J/Psi (no mass)
\newcommand{\Z}{\ensuremath{\cmsSymbolFace{Z}}\xspace} % plain Z (no superscript 0)

% Extensions for missing names in PENNAMES % note no xspace, to match syntax in PENNAMES
\newcommand{\cPgn}{\ensuremath{\nu}} % generic neutrino
\providecommand{\Pgn}{\ensuremath{\nu}} % generic neutrino
\newcommand{\cPagn}{\ensuremath{\overline{\nu}}} % generic neutrino
\providecommand{\Pagn}{\ensuremath{\overline{\nu}}} % generic neutrino
\newcommand{\cPgg}{\ensuremath{\gamma}} % gamma
\newcommand{\cPJgy}{\ensuremath{\cmsSymbolFace{J}\hspace{-.08em}/\hspace{-.14em}\psi}} % J/Psi (no mass)
\newcommand{\cPZ}{\ensuremath{\cmsSymbolFace{Z}}} % plain Z (no superscript 0)
\newcommand{\cPZpr}{\ensuremath{\cmsSymbolFace{Z}^\prime}} % plain Z'
\newcommand{\cPqt}{\ensuremath{\cmsSymbolFace{t}}} % t for t quark
\newcommand{\cPqb}{\ensuremath{\cmsSymbolFace{b}}} % b for b quark
\newcommand{\cPqc}{\ensuremath{\cmsSymbolFace{c}}} % c for c quark
\newcommand{\cPqs}{\ensuremath{\cmsSymbolFace{s}}} % s for s quark
\newcommand{\cPqu}{\ensuremath{\cmsSymbolFace{u}}} % u for u quark
\newcommand{\cPqd}{\ensuremath{\cmsSymbolFace{d}}} % d for d quark
\newcommand{\cPq}{\ensuremath{\cmsSymbolFace{q}}} % generic quark
\newcommand{\cPg}{\ensuremath{\cmsSymbolFace{g}}} % generic gluon
\newcommand{\cPG}{\ensuremath{\cmsSymbolFace{G}}} % Graviton
\newcommand{\cPaqt}{\ensuremath{\overline{\cmsSymbolFace{t}}}} % t for t anti-quark
\newcommand{\cPaqb}{\ensuremath{\overline{\cmsSymbolFace{b}}}} % b for b anti-quark
\newcommand{\cPaqc}{\ensuremath{\overline{\cmsSymbolFace{c}}}} % c for c anti-quark
\newcommand{\cPaqs}{\ensuremath{\overline{\cmsSymbolFace{s}}}} % s for s anti-quark
\newcommand{\cPaqu}{\ensuremath{\overline{\cmsSymbolFace{u}}}} % u for u anti-quark
\newcommand{\cPaqd}{\ensuremath{\overline{\cmsSymbolFace{d}}}} % d for d anti-quark
\newcommand{\cPaq}{\ensuremath{\overline{\cmsSymbolFace{q}}}} % generic anti-quark
\newcommand{\cPKstz}{\ensuremath{\cmsSymbolFace{K}^{\ast0}}\xspace} %note has xspace
% future symbols from heppennames2
\providecommand{\PH}{\ensuremath{\cmsSymbolFace{H}}\xspace} % plain Higgs
\providecommand{\Ph}{\ensuremath{\cmsSymbolFace{h}}\xspace} % SUSY Higgs
\providecommand{\PJGy}{\ensuremath{\cmsSymbolFace{J}\hspace{-.08em}/\hspace{-.14em}\psi}\xspace} % J/Psi (no mass)
\providecommand{\PBzs}{\ensuremath{\cmsSymbolFace{B}^0_\cmsSymbolFace{s}}\xspace} % B^0_s
\providecommand{\Pg}{\ensuremath{\cmsSymbolFace{g}}\xspace} % generic gluon
\providecommand{\PSg}{\ensuremath{\widetilde{\cmsSymbolFace{g}}}\xspace} % gluino
\providecommand{\PSQ}{\ensuremath{\widetilde{\cmsSymbolFace{q}}}\xspace} % squark
\providecommand{\PXXG}{\ensuremath{\cmsSymbolFace{G}}\xspace} % graviton
\providecommand{\PXXSG}{\ensuremath{\widetilde{\PXXG}}\xspace} % gravitino
\providecommand{\PSGcp}{\ensuremath{\widetilde{\chi}^+}\xspace}
\providecommand{\PSGc}{\ensuremath{\widetilde{\chi}}\xspace} % neutralino
\providecommand{\PSGcz}{\ensuremath{\widetilde{\chi}^0}\xspace} % neutralino with superscript 0
\providecommand{\PSGczDo}{\ensuremath{\widetilde{\chi}^{0}_{1}}\xspace} % neutralino
\providecommand{\PSGczDt}{\ensuremath{\widetilde{\chi}^{0}_{2}}\xspace} % neutralino
\providecommand{\PSGcpm}{\ensuremath{\widetilde{\chi}^\pm}\xspace} % neutralino
\providecommand{\PSGcpDo}{\ensuremath{\widetilde{\chi}^{+}_{1}}\xspace} % neutralino
\providecommand{\Pl}{\ensuremath{\cmsSymbolFace{l}}\xspace} % non-ell lepton
\providecommand{\PAl}{\ensuremath{\overline{\cmsSymbolFace{l}}}\xspace} % non-ell anti-lepton
\providecommand{\PGnl}{\ensuremath{\nu_\cmsSymbolFace{l}}\xspace} % lepton neutrino
\providecommand{\PAGnl}{\ensuremath{\overline{\nu}_\cmsSymbolFace{l}}\xspace} % anti-lepton neutrino
\providecommand{\PQtpr}{\ensuremath{\cmsSymbolFace{t}^{\prime}}\xspace} % t'
\providecommand{\PAQtpr}{\ensuremath{\bar{\cmsSymbolFace{t}}^\prime}\xspace} % t'-bar; needs to be converted to overline-requires rework a la heppennames
\providecommand{\PQbpr}{\ensuremath{\cmsSymbolFace{b}^{\prime}}\xspace} % b'
\providecommand{\PAQbpr}{\ensuremath{\bar{\cmsSymbolFace{b}}^\prime}\xspace} % b'-bar; needs same as anti-t'
\providecommand{\PGg}{\ensuremath{\gamma}\xspace} % gamma
\providecommand{\PKzS}{\ensuremath{\cmsSymbolFace{K}^0_\cmsSymbolFace{S}}\xspace} % K short
\providecommand{\PBs}{\ensuremath{\cmsSymbolFace{B}_\cmsSymbolFace{s}}\xspace} % B sub s
\providecommand{\PASQt}{\ensuremath{\overline{\widetilde{\cmsSymbolFace{t}}}}\xspace} % stop
\providecommand{\PSQt}{\ensuremath{\widetilde{\cmsSymbolFace{t}}}\xspace} % stop
\providecommand{\PSGt}{\ensuremath{\widetilde{\tau}}\xspace} % stau
\providecommand{\PZpr}{\ensuremath{\cmsSymbolFace{Z}^\prime}\xspace} % plain Z' using prime
\providecommand{\PW}{\ensuremath{\cmsSymbolFace{W}}\xspace} % use prime like pennames2
\providecommand{\PGn}{\ensuremath{\nu}\xspace} % generic neutrino
\providecommand{\PAGn}{\ensuremath{\overline{\nu}}\xspace} % generic neutrino
\providecommand{\PSQtDo}{\ensuremath{\widetilde{\cmsSymbolFace{t}}_1}\xspace}
\providecommand{\PSQtDt}{\ensuremath{\widetilde{\cmsSymbolFace{t}}_2}\xspace}
\providecommand{\PQt}{\ensuremath{\cmsSymbolFace{t}}\xspace} % t
\providecommand{\PAQt}{\ensuremath{\overline{\cmsSymbolFace{t}}}\xspace} %
\providecommand{\PQb}{\ensuremath{\cmsSymbolFace{b}}\xspace} % t
\providecommand{\PAQb}{\ensuremath{\overline{\cmsSymbolFace{b}}}\xspace} %


% for APS style tables
%\ifthenelse{\boolean{cms@external}}{%
%\newenvironment{scotch}[1]{\protect\centering\ruledtabular\tabular{#1}}{\endtabular\endruledtabular}
%}{
%\newenvironment{scotch}[1]{\protect\centering\tabular{#1}\hline\hline}{\hline\endtabular}
%}

% SM (still to be classified)

\newcommand{\AFB}{\ensuremath{A_\text{FB}}\xspace}
\newcommand{\wangle}{\ensuremath{\sin^{2}\theta_{\text{eff}}^\text{lept}(M^2_{\Z})}\xspace}
\newcommand{\stat}{\ensuremath{\,\text{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\,\text{(syst)}}\xspace}
\newcommand{\thy}{\ensuremath{\,\text{(theo)}}\xspace}
\newcommand{\lum}{\ensuremath{\,\text{(lumi)}}\xspace}
\newcommand{\kt}{\ensuremath{k_{\mathrm{T}}}\xspace}

\newcommand{\BC}{\ensuremath{\cmsSymbolFace{B_{c}}}\xspace}
\newcommand{\bbarc}{\ensuremath{\cPqb\cPaqc}\xspace}
\newcommand{\bbbar}{\ensuremath{\cPqb\cPaqb}\xspace}
\newcommand{\ccbar}{\ensuremath{\cPqc\cPaqc}\xspace}
\newcommand{\bspsiphi}{\ensuremath{\cmsSymbolFace{B_s} \to \JPsi\, \phi}\xspace}
\newcommand{\EE}{\ensuremath{\Pep\Pem}\xspace}
\newcommand{\MM}{\ensuremath{\Pgmp\Pgmm}\xspace}
\newcommand{\TT}{\ensuremath{\Pgt^{+}\Pgt^{-}}\xspace}

\newcommand{\Pp}{\ensuremath{{p}}}

%%%  E-gamma definitions
\newcommand{\HGG}{\ensuremath{\cmsSymbolFace{H}\to\gamma\gamma}}
\newcommand{\GAMJET}{\ensuremath{\gamma + \text{jet}}}
\newcommand{\PPTOJETS}{\ensuremath{\Pp\Pp\to\text{jets}}}
\newcommand{\PPTOGG}{\ensuremath{\Pp\Pp\to\gamma\gamma}}
\newcommand{\PPTOGAMJET}{\ensuremath{\Pp\Pp\to\gamma + \mathrm{jet}}}
\newcommand{\MH}{\ensuremath{M_{\PH}}}
\newcommand{\RNINE}{\ensuremath{R_\mathrm{9}}}
\newcommand{\DR}{\ensuremath{\Delta R}}





%%%%%%
% From Albert
%

\newcommand{\ga}{\ensuremath{\gtrsim}}
\newcommand{\la}{\ensuremath{\lesssim}}
%
\newcommand{\swsq}{\ensuremath{\sin^2\theta_\cmsSymbolFace{W}}\xspace}
\newcommand{\cwsq}{\ensuremath{\cos^2\theta_\cmsSymbolFace{W}}\xspace}
\newcommand{\tanb}{\ensuremath{\tan\beta}\xspace}
\newcommand{\tanbsq}{\ensuremath{\tan^{2}\beta}\xspace}
\newcommand{\sidb}{\ensuremath{\sin 2\beta}\xspace}
\newcommand{\alpS}{\ensuremath{\alpha_S}\xspace}
\newcommand{\alpt}{\ensuremath{\tilde{\alpha}}\xspace}

\newcommand{\QL}{\ensuremath{\cmsSymbolFace{Q}_\cmsSymbolFace{L}}\xspace}
\newcommand{\sQ}{\ensuremath{\widetilde{\cmsSymbolFace{Q}}}\xspace}
\newcommand{\sQL}{\ensuremath{\widetilde{\cmsSymbolFace{Q}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\ULC}{\ensuremath{\cmsSymbolFace{U}_\cmsSymbolFace{L}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sUC}{\ensuremath{\widetilde{\cmsSymbolFace{U}}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sULC}{\ensuremath{\widetilde{\cmsSymbolFace{U}}_\cmsSymbolFace{L}^\cmsSymbolFace{C}}\xspace}
\newcommand{\DLC}{\ensuremath{\cmsSymbolFace{D}_\cmsSymbolFace{L}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sDC}{\ensuremath{\widetilde{\cmsSymbolFace{D}}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sDLC}{\ensuremath{\widetilde{\cmsSymbolFace{D}}_\cmsSymbolFace{L}^\cmsSymbolFace{C}}\xspace}
\newcommand{\LL}{\ensuremath{\cmsSymbolFace{L}_\cmsSymbolFace{L}}\xspace}
\newcommand{\sL}{\ensuremath{\widetilde{\cmsSymbolFace{L}}}\xspace}
\newcommand{\sLL}{\ensuremath{\widetilde{\cmsSymbolFace{L}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\ELC}{\ensuremath{\cmsSymbolFace{E}_\cmsSymbolFace{L}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sEC}{\ensuremath{\widetilde{\cmsSymbolFace{E}}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sELC}{\ensuremath{\widetilde{\cmsSymbolFace{E}}_\cmsSymbolFace{L}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sEL}{\ensuremath{\widetilde{\cmsSymbolFace{E}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\sER}{\ensuremath{\widetilde{\cmsSymbolFace{E}}_\cmsSymbolFace{R}}\xspace}
\newcommand{\sFer}{\ensuremath{\widetilde{\cmsSymbolFace{f}}}\xspace}
\newcommand{\sQua}{\ensuremath{\widetilde{\cmsSymbolFace{q}}}\xspace}
\newcommand{\sUp}{\ensuremath{\widetilde{\cmsSymbolFace{u}}}\xspace}
\newcommand{\suL}{\ensuremath{\widetilde{\cmsSymbolFace{u}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\suR}{\ensuremath{\widetilde{\cmsSymbolFace{u}}_\cmsSymbolFace{R}}\xspace}
\newcommand{\sDw}{\ensuremath{\widetilde{\cmsSymbolFace{d}}}\xspace}
\newcommand{\sdL}{\ensuremath{\widetilde{\cmsSymbolFace{d}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\sdR}{\ensuremath{\widetilde{\cmsSymbolFace{d}}_\cmsSymbolFace{R}}\xspace}
\newcommand{\sTop}{\ensuremath{\widetilde{\cmsSymbolFace{t}}}\xspace}
\newcommand{\stL}{\ensuremath{\widetilde{\cmsSymbolFace{t}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\stR}{\ensuremath{\widetilde{\cmsSymbolFace{t}}_\cmsSymbolFace{R}}\xspace}
\newcommand{\stone}{\ensuremath{\widetilde{\cmsSymbolFace{t}}_1}\xspace}
\newcommand{\sttwo}{\ensuremath{\widetilde{\cmsSymbolFace{t}}_2}\xspace}
\newcommand{\sBot}{\ensuremath{\widetilde{\cmsSymbolFace{b}}}\xspace}
\newcommand{\sbL}{\ensuremath{\widetilde{\cmsSymbolFace{b}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\sbR}{\ensuremath{\widetilde{\cmsSymbolFace{b}}_\cmsSymbolFace{R}}\xspace}
\newcommand{\sbone}{\ensuremath{\widetilde{\cmsSymbolFace{b}}_1}\xspace}
\newcommand{\sbtwo}{\ensuremath{\widetilde{\cmsSymbolFace{b}}_2}\xspace}
\newcommand{\sLep}{\ensuremath{\widetilde{\cmsSymbolFace{l}}}\xspace}
\newcommand{\sLepC}{\ensuremath{\widetilde{\cmsSymbolFace{l}}^\cmsSymbolFace{C}}\xspace}
\newcommand{\sEl}{\ensuremath{\widetilde{\cmsSymbolFace{e}}}\xspace}
\newcommand{\sElC}{\ensuremath{\widetilde{\cmsSymbolFace{e}}^\cmsSymbolFace{C}}\xspace}
\newcommand{\seL}{\ensuremath{\widetilde{\cmsSymbolFace{e}}_\cmsSymbolFace{L}}\xspace}
\newcommand{\seR}{\ensuremath{\widetilde{\cmsSymbolFace{e}}_\cmsSymbolFace{R}}\xspace}
\newcommand{\snL}{\ensuremath{\widetilde{\nu}_L}\xspace}
\newcommand{\sMu}{\ensuremath{\widetilde{\mu}}\xspace}
\newcommand{\sNu}{\ensuremath{\widetilde{\nu}}\xspace}
\newcommand{\sTau}{\ensuremath{\widetilde{\tau}}\xspace}
\newcommand{\Glu}{\ensuremath{\cmsSymbolFace{g}}\xspace}
\newcommand{\sGlu}{\ensuremath{\widetilde{\cmsSymbolFace{g}}}\xspace}
\newcommand{\Wpm}{\ensuremath{\cmsSymbolFace{W}^{\pm}}\xspace}
\newcommand{\sWpm}{\ensuremath{\widetilde{\cmsSymbolFace{W}}^{\pm}}\xspace}
\newcommand{\Wz}{\ensuremath{\cmsSymbolFace{W}^{0}}\xspace}
\newcommand{\sWz}{\ensuremath{\widetilde{\cmsSymbolFace{W}}^{0}}\xspace}
\newcommand{\sWino}{\ensuremath{\widetilde{\cmsSymbolFace{W}}}\xspace}
\newcommand{\Bz}{\ensuremath{\cmsSymbolFace{B}^{0}}\xspace}
\newcommand{\sBz}{\ensuremath{\widetilde{\cmsSymbolFace{B}}^{0}}\xspace}
\newcommand{\sBino}{\ensuremath{\widetilde{\cmsSymbolFace{B}}}\xspace}
\newcommand{\Zz}{\ensuremath{\cmsSymbolFace{Z}^{0}}\xspace}
\newcommand{\sZino}{\ensuremath{\widetilde{\cmsSymbolFace{Z}}^{0}}\xspace}
\newcommand{\sGam}{\ensuremath{\widetilde{\gamma}}\xspace}
\newcommand{\chiz}{\ensuremath{\widetilde{\chi}^{0}}\xspace}
\newcommand{\chip}{\ensuremath{\widetilde{\chi}^{+}}\xspace}
\newcommand{\chim}{\ensuremath{\widetilde{\chi}^{-}}\xspace}
\newcommand{\chipm}{\ensuremath{\widetilde{\chi}^{\pm}}\xspace}
\newcommand{\Hone}{\ensuremath{\cmsSymbolFace{H}_\cmsSymbolFace{d}}\xspace}
\newcommand{\sHone}{\ensuremath{\widetilde{\cmsSymbolFace{H}}_\cmsSymbolFace{d}}\xspace}
\newcommand{\Htwo}{\ensuremath{\cmsSymbolFace{H}_\cmsSymbolFace{u}}\xspace}
\newcommand{\sHtwo}{\ensuremath{\widetilde{\cmsSymbolFace{H}}_\cmsSymbolFace{u}}\xspace}
\newcommand{\sHig}{\ensuremath{\widetilde{\cmsSymbolFace{H}}}\xspace}
\newcommand{\sHa}{\ensuremath{\widetilde{\cmsSymbolFace{H}}_\cmsSymbolFace{a}}\xspace}
\newcommand{\sHb}{\ensuremath{\widetilde{\cmsSymbolFace{H}}_\cmsSymbolFace{b}}\xspace}
\newcommand{\sHpm}{\ensuremath{\widetilde{\cmsSymbolFace{H}}^{\pm}}\xspace}
\newcommand{\hz}{\ensuremath{\cmsSymbolFace{h}^{0}}\xspace}
\newcommand{\Hz}{\ensuremath{\cmsSymbolFace{H}^{0}}\xspace}
\newcommand{\Az}{\ensuremath{\cmsSymbolFace{A}^{0}}\xspace}
\newcommand{\Hpm}{\ensuremath{\cmsSymbolFace{H}^{\pm}}\xspace}
\newcommand{\sGra}{\ensuremath{\widetilde{\cmsSymbolFace{G}}}\xspace}
%
\newcommand{\mtil}{\ensuremath{\widetilde{m}}\xspace}
%
\newcommand{\rpv}{\ensuremath{\rlap{\kern.2em/}R}\xspace}
\newcommand{\LLE}{\ensuremath{LL\bar{E}}\xspace}
\newcommand{\LQD}{\ensuremath{LQ\bar{D}}\xspace}
\newcommand{\UDD}{\ensuremath{\overline{UDD}}\xspace}
\newcommand{\Lam}{\ensuremath{\lambda}\xspace}
\newcommand{\Lamp}{\ensuremath{\lambda'}\xspace}
\newcommand{\Lampp}{\ensuremath{\lambda''}\xspace}
%
\newcommand{\spinbd}[2]{\ensuremath{\bar{#1}_{\dot{#2}}}\xspace}

\newcommand{\MD}{\ensuremath{{M_\mathrm{D}}}\xspace}% ED mass
\newcommand{\Mpl}{\ensuremath{{M_\mathrm{Pl}}}\xspace}% Planck mass
\newcommand{\Rinv} {\ensuremath{{R}^{-1}}\xspace}
\endinput

